SMaLL: A Software Framework for portable Machine Learning Libraries

Interest in deploying Deep Neural Network (DNN) inference on edge devices has resulted in an explosion of the number and types of hardware platforms to use. While the high-level programming interface, such as TensorFlow, can be readily ported across different devices, high-performance inference implementations rely on a good mapping of the high-level interface to the target hardware platform. Commonly, this mapping may use optimizing compilers to generate code at compile time or high-performance vendor libraries that have been specialized to the target platform. Both approaches rely on expert knowledge to produce the mapping, which may be time-consuming and difficult to extend to new architectures. In this work, we present a DNN library framework, SMaLL, that is easily extensible to new architectures. The framework uses a unified loop structure and shared, cache-friendly data format across all intermediate layers, eliminating the time and memory overheads incurred by data transformation between layers. Layers are implemented by simply specifying the layer's dimensions and a kernel -- the key computing operations of each layer. The unified loop structure and kernel abstraction allows us to reuse code across layers and computing platforms. New architectures only require the 100s of lines in the kernel to be redesigned. To show the benefits of our approach, we have developed software that supports a range of layer types and computing platforms, which is easily extensible for rapidly instantiating high performance DNN libraries. We evaluate our software by instantiating networks from the TinyMLPerf benchmark suite on 5 ARM platforms and 1 x86 platform ( an AMD Zen 2). Our framework shows end-to-end performance that is comparable to or better than ML Frameworks such as TensorFlow, TVM and LibTorch.

==> FrameworkDesign.tex <==
\section{Framework Design}


==> FutureWork.tex <==
% Should these use a python frontend interface?  Integrate using tensorflow OP?
% Code gen/parser for ONNX-SMaLL. MLIR.
% Fusion passes.
% extending to GPUs/accelerators.

% ideas:
% - creating a python module for small
% - Adding SMaLL dialect to MLIR
% - Adding a converter from ONNX to SMaLL via MLIR
% - Creating a SMall-opt tool to perform fusion automatically
% - Creating kernels for the Jetson/Xavier GPUs
% - Adding more architectures to SMaLL



\subsection{Ease of Architectural Portability}


\subsection{Network-aware optimizations}
Cross layer optimization. Resnet skip layers, fusion activation. Better Parallelization



% \subsection{Usability}
% Github repo
% Secondly, we would like to allow users of other machine learning frameworks to be able to easily convert their models into SMaLL.
% We also are looking into leveraging the MLIR compiler infrastructure~\cite{mlir}. Our goal is to design an MLIR dialect for SMaLL such that we can create an optimizer driver and code gen tools. With the optimizer driver we are looking to perform optimizations automatically such as loop fusion. Furthermore, we are considering using our SMaLL MLIR dialect to automatically generate high performing code for new architectures, similar to PolyDL~\cite{polydl}. 




==> RelatedWork.tex <==



%\subsection{ML Frameworks}
%Tensorflow+XLA\\
%libtorch / pytorch\\
%\subsection{High Performance ML Backends}
CMSIS-NN \\
OneDNN\\

\subsection{Runtime ML Libraries}
TFlite\\
glow


==> figures/gen_conv.tex <==
\begin{algorithm}
\caption{Loops For a Generalized DNN Operation}\label{alg:gen_conv}
\begin{algorithmic}[1]
\For {$g \leq G$}
    \For {$j \leq K$}
        \For {$k \leq O_{h}$}
            \For {$l \leq O_{w}$}
                \For {$x \leq F_{h}$}
                    \For {$y \leq F_{w}$}
                        \For {$i \leq F_C$}
                            % \State{$ReductionOperator$(}
                            % \State{$\quad O_{[gK + j][k][l]}$}
                            % \State{$\quad I_{[(gF_C)\times S_{C} + i][k\times S_{H} + x ][l \times S_{W} + y]} $}
                            % \State{$\quad F_{[gK + j][i][x][y]}$}
                            \State{{ReductionOp($O, W, I, s_H, s_W, s_C$)}}
%                         \EndFor
%                     \EndFor
%                 \EndFor
%             \EndFor
%         \EndFor
%     \EndFor
% \EndFor


\end{algorithmic}
\end{algorithm}



==> figures/kernel_structure.tex <==
\color{black}
\begin{algorithm}
\caption{Kernel for Full Channel Reduction}\label{alg:kernel}
\begin{algorithmic}[1]
\For{$g \leq G$ in parallel}
    \For {$j \leq K$ in parallel}\label{channel_block}
     \State{}
        \For {$i \leq F_C $}
        \State{}
        \color{black}
          \For {$k \leq O_{h}$}\label{height} 
          \color{black}
                \For {$l \leq O_{w}$} \label{pixel_block}
                    \For {$x \leq F_{h}$} 
                        \For {$y \leq F_{w}$}
                            \For {$ii\leq I_{cb}$}
                                \For {$ll \leq O_{wb}$} \label{pixels}
                                    \For {$jj \leq O_{cb}$}\label{channels}       
                                        \State{ReductionOp($O_0, I, F_0$)}       
\end{algorithmic}
\end{algorithm}

==> figures/reduction_op.tex <==
\begin{algorithm}
\caption{Specification  of the abstract reduction operation for a Convolution }\label{alg:fma_reduction_op}
\begin{algorithmic}[1]
\Function{ReductionOp\_FMA}{$O, W, I, s_H, s_W, s_C$}
    \State{$\quad O[g][k][j][l] += I[(gF_C)\cdot S_{C} + i][k\cdot S_{H} + x ][l \cdot S_{W} + y] \times
    W[g][k][x][y]$}
\EndFunction
\end{algorithmic}
\end{algorithm}


==> figures/table_combined.tex <==
\begin{table}[h!]
\centering

    \begin{tabular}{lllp{15mm}p{20mm}l}
        \hline \hline
        Class & Layer Type & Filter Dims & Batch Dims & Stride Dims & Kernel\\
        \hline
        Single Element & Activation (ReLU)& \{1, 1, 1\} &$\{1, G\}$&$\{1, 1, 1\}$ & Max\\
        &        Batch Normalization& \{1, 1, 1\} &$\{1,G\}$&$\{1, 1, 1\}$ & FMA  \\
         &        Upsample& \{1, 1, 1\} &$\{1,G\}$&$\{S_H, S_W, 1\}$ & Assignment \\

                
        Single Channel &  Depthwise Convolutions &$\{F_H, F_W, 1\}$&$\{1, G\}$& $\{S_H, S_W, 1\}$ &  E-wise FMA\\
                       & Max Pooling& $\{F_H, F_W, 1\}$&$\{1, G\}$& $\{S_H, S_W, 1\}$ & Max \\
        Partial Channel &  Group Convolutions & $\{F_H, F_W, F_C\}$&$\{K, G\}$&$\{S_H, S_W, F_C\}$ & FMA \\
Full Channel &Convolution &$\{F_H, F_W, I_C\}$& $\{K, 1\}$&$\{ S_H, S_W, 1\}$ & FMA \\
        & Bottleneck($1\times 1$ Convolution)& $\{1, 1, I_C\}$&$\{K, 1\}$&$\{S_H, S_W, 1\}$ & FMA \\
        & Fully Connected  &  $\{I_H, I_W, I_C\}$&$\{K, 1\}$&$\{1, 1, 1\}$ & FMA* \\       
%        Full Spatial & Global Average Pooling & $\{I_H, I_W, 1\}$ &$\{1, G\}$&$\{1, 1, 1\}$ \\
        % \verb|               (scale)|& $O *= F$ &$\{1, 1, 1\}$ &$\{1, N\}$&$\{1, 1, 1\}$ \\
        \hline \hline
    \end{tabular}
\caption{List of Currently Supported Machine Learning Layers. Dialation is set to 1}
\label{tab:loop_mapping}

\end{table}



